Automated Performance Testing Based on Active Deep Learning

Generating tests that can reveal performance issues in large and complex software systems within a reasonable amount of time is a challenging task. On one hand, there are numerous combinations of input data values to explore. On the other hand, we have a limited test budget to execute tests. What makes this task even more difficult is the lack of access to source code and the internal details of these systems. In this paper, we present an automated test generation method called ACTA for black-box performance testing. ACTA is based on active learning, which means that it does not require a large set of historical test data to learn about the performance characteristics of the system under test. Instead, it dynamically chooses the tests to execute using uncertainty sampling. ACTA relies on a conditional variant of generative adversarial networks,and facilitates specifying performance requirements in terms of conditions and generating tests that address those conditions.We have evaluated ACTA on a benchmark web application, and the experimental results indicate that this method is comparable with random testing, and two other machine learning methods,i.e. PerfXRL and DN.

==> sections/2-Example.tex <==
ABB is a leading supplier of industrial robots and robot software. As shown in Figure \ref{fig:example}, the heart of each robotic solution offered by ABB is a controller software developed with the RAPID language. RAPID is a flexible and powerful language for developing modular and multi-tasking robot applications. Currently, the performance of RAPID programs is tested manually using TCs developed by RAPID programmers. However, due to the increasing complexity and diversity of the produced robots and the services requested by customers, the need for automating the performance testing process is highlighted recently.

\begin{figure*}[bht]
\centerline{\includegraphics[width=\textwidth]{figures/example.pdf}}

\caption{Manual testing of robotic software in ABB.}

\label{fig:example}
\end{figure*}

In the manual testing process, several tests have to be executed upon each change in the operating system, hardware or the RAPID program. Not only, the manual process is time-consuming and laborious, but also it is error-prone and does not provide any correctness guarantee since it relies on human knowledge. Taking advantage of the recent advances in machine learning, \method is capable of learning from the SUT while generating positive tests automatically. 

For illustration purposes, we consider a simple RAPID program implementing a movement scenario. Target position, motion speed and zone, and hardware configuration file are the input parameters that we use to generate tests. The goal is to find a combination of input values for these parameters that will lead to a performance issue when applied to the movement scenario. The performance measures to be evaluated on each execution of the scenario include...


